The Impact of DNS Insecurity on Time

We demonstrate the first practical off-path time shifting attacks against NTP as well as against Man-in-the-Middle (MitM) secure Chronos-enhanced NTP. Our attacks exploit the insecurity of DNS allowing us to redirect the NTP clients to attacker controlled servers. We perform large scale measurements of the attack surface in NTP clients and demonstrate the threats to NTP due to vulnerable DNS.

==> ntp-old.tex <==
\section{Introduction}
\label{sc:ntp}

Network Time Protocol (NTP) uses DNS for querying upstream servers for time synchronisation, which the local NTP server then provides to hosts on its network.



\subsection{Measurement Methodology}

We evaluated vulnerabilities in popular NTP implementations against DNS-based attacks (see Table \ref{tab:ntpclients}) by triggering queries using both boot-time and run-time configurations. We found that all NTP implementations are vulnerable to cache poisoning at boot-time when performing DNS lookups. An exception to this is a hardened Chronos NTP implementation \cite{ntp:chronos} which performs DNS lookups once at installation time. However, since targeting boot-time configuration requires predicting when an NTP server is booting using some side channel, we measured the attack surface considering only run-time configuration. Since most tested NTP servers do not issue DNS queries at run-time, our attack first requires disrupting the existing associations with upstream NTP servers. To do so, the attacker needs to know the addresses of the upstream NTP servers currently being used by the target NTP server. This can be done in a number of ways:
\\
\textbf{1. Listing IP addresses of upstream NTP servers present in the pool:} The attacker attempts to resolve the hostnames configured in an NTP server and creates a list of possible upstream NTP server addresses. For the \texttt{pool.ntp.org} server pool, the list consists of 2000-3000 servers, which is small enough for the attacker to successfully disrupt existing associations with any of these servers by abusing NTP's rate limiting mechanism.
\\
\textbf{2. Leakage of upstream NTP server's IP address:} An NTP host typically acts as an NTP client and NTP server at the same time (\textit{ntpd}'s default configuration). Thus, an attacker can query the (local) NTP server for which the server sends back a response that contains the `Reference ID' field. This field represents the IP address of the upstream NTP server to which the local NTP server is synchronised.  In this case, the attacker learns only one server address at a time and thus, needs to wait until the upstream server is changed.
\\
\textbf{3. Using NTP control queries:} Some NTP servers respond to NTP control queries and expose the NTP configuration details which can be used to learn both, the configured DNS hostnames as well as all currently used upstream NTP server's IP addresses. We found that 5.3 \% of the NTP servers in the \texttt{pool.ntp.org} pool respond to configuration queries.

\section{Attack Overview}

There are two ways to attack NTP via DNS cache poisoning: \textit{Indirect} and \textit{Direct}. {\em Indirect} assumes that the DNS resolver used by NTP is also used by another service which can be used to trigger DNS queries and to perform cache poisoning. The attacker uses that other service to perform DNS cache poisoning and then redirects NTP communication to an attacker's host. {\em Direct} assumes that no other service is using the DNS resolver except for an NTP server, and the cache poisoning attack has to be performed via the NTP server directly.

\subsubsection{Direct attacks against NTP}

How and when the NTP server issues a DNS request depends on the upstream server configuration. Upstream server configuration can be typically done in 2 ways depending on the used client: 

{\bf Single server configuration.} The client is given a list of DNS hostnames, which are then resolved once at boot-time. 

{\bf Pool server configuration.} The client resolves each hostname multiple times whenever new NTP server addresses are needed.




Depending on the configuration two approaches for triggering DNS requests for poisoning attack are possible:
\begin{figure}[ht!]
    \centering
    \includegraphics[width=8cm]{img/ntp-flow.pdf}
    \caption{Simplified attack on ntpd.}
    \label{fig:ntp_sequence_diagram}
\end{figure}

{\bf DNS requests at boot-time.} During client startup, the attacker poisons the DNS request for the {\it pool.ntp.org}. Unless the attacker has side channel allowing it to predict when the NTP server boots, it has to be a MitM between local NTP server and NTP upstream server. 

{\bf DNS requests at run-time.} During runtime, a local NTP server typically has a list of NTP servers resolved as IP addresses. Nevertheless, the attacker can force the local NTP server to perform DNS lookups by disturbing the communication to one or more NTP servers. This will cause the local NTP server to replace the unreachable servers. To hinder the association to existing NTP servers, an attacker can abuse the NTP's rate limiting mechanism, which works as follows:

To prevent reflection-based denial of service attacks, NTP servers employ rate-limiting for requests. This causes the server
to stop sending replies if too many requests are received from the same IP address in a certain time-frame (normally the limit is in the range of 1 request/second). An attacker can abuse the rate limiting mechanism by continuously sending spoofed NTP requests with the client's IP address. This in turn causes the server to stop
responding to the clients requests. Through experimental evaluation we found that $38\%$ of the servers in the \texttt{pool.ntp.org} pool support rate limiting.


{\bf Attack steps.} A simplified run-time attack against a local NTP server with only a single upstream NTP server is illustrated in Figure \ref{fig:ntp_sequence_diagram}. For simplicity we refer to a local NTP server - NTP client and to upstream NTP server - NTP upstream. At ``Client startup'', the NTP client requests an \texttt{A} record for \texttt{pool.ntp.org} and sets up an association to the server at \texttt{1.1.1.1}. After a while, the attacker decides to start the attack, which is marked by the ``Attack starts'' mark. First he poisons the NTP client's resolver with an \texttt{A} record for \texttt{pool.ntp.org} with the address \texttt{6.6.6.6}, which is controlled by the attacker. After that, he sends an NTP request to the NTP client and the client answers with an NTP response, which leaks the address of the currently used upstream NTP server at \texttt{1.1.1.1}. Now that the attacker knows the upstream server's address, he starts sending spoofed NTP requests to \texttt{1.1.1.1} with source address set to that of the NTP client. After some requests, the upstream NTP server's rate-limiting mechanism kicks in which triggers sending of a so-called ``Kiss-o-Death'' (KoD) packet to the NTP client, indicating it should query the server at a lower rate. After that, the upstream server stops answering requests with source address \texttt{1.1.1.1}, so any request from the NTP client will be unanswered. After 8 unanswered NTP requests, the NTP client will mark the upstream NTP server as unresponsive and will try to replace it using the configured DNS pool. Because of the previously poisoned cache, the NTP client will get the IP address \texttt{6.6.6.6} as an answer to its request for \texttt{pool.ntp.org IN A?}. Finally, the NTP client sets up a new association using the attacker as it's new upstream NTP server.

\subsubsection{Indirect attacks against NTP} Although attackers can cause the local NTP servers to issue DNS requests, it requires effort and preparation on behalf of the attacker. We show that in practice, due to existence of other systems and protocols, it is much easier to attack NTP ``indirectly''. Specifically, in typical network configurations, multiple servers use the same DNS resolvers for lookup services, e.g., NTP and Email servers. Our idea is to use another server, say Email server, that uses the same DNS resolver as the victim NTP server, to trigger DNS requests easily and hence be able to control the attack and the setup precisely.

The attacker uses the Email server to poison the DNS cache: inject a malicious record mapping the NTP nameserver to a host controlled by the attacker. Upon NTP requests from local NTP server the attacker returns incorrect time.

\subsection{Discussion}
One of the significant issues with NTP is usage of DNS resolvers shared with other services, which allows to attack NTP indirectly.


Notice, even security proposals for NTP which do not take into account the Internet ecosystem, where protocols depend on other systems, do not guarantee security. For instance, to mitigate NTP's problems with MitM-attackers, \cite{ntp:chronos} proposed Chronos: an NTP client which uses a large pool of servers to prevent MitM attacks. While the design of \cite{ntp:chronos} even
includes a theoretical proof of security, it relies heavily on the method it uses to generate the pool of servers and does not reflect the Internet ecosystem where NTP servers run in practice. The proposed implementation does this by querying the
\texttt{pool.ntp.org} domain every hour for 24 hours and uses the union of the resulting IP address sets as the server pool. However, even an off-path attacker that poisons the DNS cache injecting a malicious record redirecting {\it pool.ntp.org} to an attacker's controlled IP address can subvert Chronos. Subsequently, the attacker can simply provide a large amount of attacker controlled IP addresses in the pool. Using our techniques for cache poisoning, an {\bf off-path attacker} can subvert the security of Chronos which was designed to be secure even against MitM attackers.




    
    
        
        













==> rebuttal.tex <==
We thank the reviewers for the thoughtful and constructive comments on our submission. We agree with the requested changes and are working on integrating them into our manuscript. Responses to reviewers comments:

Our work uses some known techniques in new ways to launch attacks against NTP. We also devise new methodologies for triggering and predicting DNS requests. NTP was believed to be secure against off-path attackers and Chronos NTP was devised to be secure against on-path attackers. We show that both are vulnerable even to our weak off-path attackers (let alone to stronger, e.g., BGP hijacking, attackers which are common in practice). This is in contrast to [2] which constructed Chronos to be secure even against on-path (MtiM) attackers. Nevertheless, our attacks are possible since Chronos assumes guarantees from DNS, which DNS was not designed to guarantee. We demonstrate that the assumptions that Chronos is based on do not hold in practice. We devise methodologies allowing off-path attackers to predict or trigger queries and time their attack accordingly. We perform measurements and experimental evaluation of the attack. Our work is similar to other attacks which leverage known techniques and show security implications for systems which were believed to be secure, e.g., traffic analysis attacks against web communication, side channels in clouds to attack other tenants.

[boot-time attack.] There are three ways to carry out the cache poisoning attack at boot-time: (1) by predicting the time of the query via side channels, (2) by causing other systems that use the DNS resolver, such as Email or open resolver, to issue the query, or (3) by periodically planting the spoofed (second) fragments in the IP defrag. cache of the victim resolver (in payload of each fragment there is the malicious record mapping legitimate NTP servers to attacker's IP addresses), until the resolver issues the target query.

Since our main goal was to demonstrate feasibility of practical off-path attacks against NTP, to save space we removed the other methodologies (2) and (3). We briefly describe (2) and (3) next and will add an explanation as well as our measurements to the manuscript. In (2), the attacker can use other systems (like, Web, Email, or open Resolvers) to issue the query. For instance, consider using the Email server to cause the DNS resolver to issue the DNS request. The idea is to send an Email to the target domain - this causes the DNS resolver to initiate queries for SPF/TXT/DKIM/DMARC/PTR records for anti-spam mechanisms as well as for MX/A records for identifying the sending Email server, e.g., to send error messages (DSN) in case the recipient does not exist. Our measurements demonstrated that more than 70%

(3) Replanting spoofed fragment: the attacker sends the spoofed 2nd fragment every 30secs (corresponding to the time the fragment stays in the cache) until the query is issued by the resolver. Then, the response from the nameserver is sent and the first fragment of the response will be reassembled with the second fragment of the attacker that is waiting in the IP defrag. cache. As a result, the query from the victim NTP client arrives at attacker's NTP server - hence signalling to the attacker that the attack succeeded. This requires the attacker to send one spoofed fragment to the resolver's IP defrag cache at most once in every 30 seconds, corresponding to the fragment reassembly timeout. We measured frag. reassembly timeout of 60 to 120 seconds on Windows distributions and 30 seconds on Linux; [RFC2460] specifies the reassembly timeout of 60 seconds. This approach requires a low attack volume which can be completed with only one low bandwidth attacking host. Furthermore, the TTL of pool.ntp.org A record is only 150 sec. Namely, the resolver will frequently issue queries for pool.ntp.org, at most every 150 sec. This means that the attacker needs to maintain the spoofed fragment in the IP defrag. cache for at most 150 sec, which in the worst case requires 150/30 = 5 spoofed (second) fragments per attack.

[DNSSEC.] We will integrate discussion on DNSSEC, and the problems at the start of the manuscript. Currently none of the servers in pool.ntp.org support DNSSEC. Even a fully deployed DNSSEC would not always prevent our attack, e.g., due to errors or misconfigurations, [35] showed that vulnerable key generation&management practices render signed domains vulnerable to attacks.

[Not NTP's vulnerability.] The systems in the Internet run concurrently with other systems and depend on other Internet protocols and systems for performance and correctness. Hence security of the Internet components cannot be analysed in isolation from the rest of the Internet. Although the community believes NTP to be secure, in practice NTP servers do not use any security features. Hence carrying out the attacks in practice is critical for demonstrating the risks and avoiding illusion of security.

[pool.ntp.org is often cached.] First, the record is cached for at most 150sec (as set in TTL of pool.ntp.org). Second, via a measurement study we found that the resolvers are used by different services concurrently, e.g., NTP server, Web and Email server (we will add explanation to paper). Therefore, the attacker can leverage other systems to trigger queries or evict cached records from the cache (e.g., by filling the cache with junk records, it causes the least recently used records to be evicted). The attacker can also use a different strategy, e.g., attack NS (nameserver records) instead of NTP server records, and hijack the entire domain instead of just NTP service. Using other services enables the attacker to also query different subdomains of the target domain.

 [Measurements in residential networks.] We presented two methods to perform measurements in DNS resolvers residential networks in the paper: via RD=0 and via latency measurements. As we showed, to improve accuracy of latency measurements more traffic as well as eviction of the cached records are needed. We avoided tests that could harm performance of the networks in the Internet and low traffic volume was sufficient to show practicality of the attack (even the tests with the open resolvers use the minimal possible traffic volume at the cost of sacrificing accuracy). 

[Rate limit in NTP servers.] 38\% of servers in pool.ntp.org enforce rate limiting (Section VII in paper).

[Roughtime/NTS] are currently IETF drafts, that were not reviewed/standardised by the community, e.g., they may have introduce new/other vulnerabilities or problems which were not yet reviewed/evaluated by the community, or may have deployment issues preventing their adoption in the Internet, e.g., due to the significant changes that they require to the NTP ecosystem (indeed, in our measurements we have not identified a single server supporting them).

[Percentage of hosts vulnerable.] Our goal was to demonstrate practicality of our attacks and to show that the problem is not a bug in a single system, but an inherent issue in the design. We did so, while keeping the attack traffic low in order not to intervene with the performance of the measured networks/servers. Increasing the traffic or using multiple attacking hosts increases the coverage of the vulnerable hosts. Nevertheless, even in that limited mode we found more vulnerable hosts than the prior work of [1] (which found that potentially 0,0008%
- all NTP implementations are vulnerable to boot-time-attack
- 4/7 NTP implementations are vulnerable to run-time attack, with market share data from [29] we get that 4/7 is 45%
(see manuscript, table I)

Our study of clients in the wild yielded: 
- 32%
- 91%


[Evaluation analysis not enough/not detailed.] We will add an explanation and more examples of different configurations and their implications for NTP clients.

[MTU sizes in popular nameservers.] The minimum MTU sizes that we managed to reduce in nameservers are as follows (we will also add to the paper)
- 296 or lower: 16%
- 600 or lower: 80%


Our message is that doing so leads to vulnerabilities, and we demonstrate one such attack which exploits DNS. Our attack uses the weakest off-path attacker and demonstrates a vulnerability in plain NTP and for enhanced NTP with Chronos - of course such attacks are much easier to launch with a stronger attacker, such as BGP prefix hijacking attacker, which is common in the Internet. 

We tested our methodology in the lab and it works as follows: our probers issue queries to the resolvers in residential networks, asking for IP addresses of NTP servers, and measure the time that it takes to receive the response. When the DNS resolver has records in cache - it would not need to query the nameservers in the Internet. Hence the latency to receive responses is equivalent to the latency to the resolver and back to our prober. When the resolver does not have the records in the cache, it would go and query the nameservers in the Internet, hence increasing the latency with an additional RTT (round trip time) to the nameserver and back to the resolver + the latency from our prober to the resolver and back. We use this to differentiate cases when the NTP record is in cache vs when it is not in cache. Notice that to ensure correctness of the results, the experiments have to be repeated multiple times - this requires evicting the cached records after the first run or overwriting them with new values, then repeating the experiment. Evicting the records harms the performance of the networks on which measurements are performed.

[The "attack duration"] in Table II is unclear,... in two scenarios the NTPd has different values. This is because NTPd can be attacked with both methods, P1 (where the attacker already konws the set of upsream NTP servers) or P2 (where the attacker discovers the upstream NTP servers one-after-another by querying the client). This is not the case for openntpd and chrony because those do not leak information about the used upstream NTP servers and so only P1 is applicable.


In our measurements the reassembly timeout in linux is set to 30 seconds and in Windows distributions between 60 and 120 seconds. The reassembly timeout is hardcoded on Windows and cannot be changed. In RFC 2460 the reassembly timeout is 60 seconds.



[Measurements in residential networks.] Performing measurements of cached records in resolvers in residential networks via an ad-network would require a large traffic volume and would require eviction of cached records by us from the caches of the resolver, hence would intervene with the performance of the resolvers on those networks. Therefore we avoided tests that could harm performance of the networks in the Internet and low traffic volume was sufficient to show practicality of the attack (even the tests with the open resolvers use the minimal possible traffic volume at the cost of sacrificing accuracy). 

==> related-work.tex <==
\section{Related work}\label{sc:works}
\label{sec:relwork}




\begin{mytodoenv}

Attacking NTP directly \\
    - Via Non-standard NTP queries, Config interface \cite{kiayias_security_2017}, vulnerabilities should be closed (however, still 5\% of NTP servers have open config) \\
    - Via Fragmentation \cite{malhotra_attacking_2016-1} theoretically possible, but needs PMTUD support for MTU=68 (unrealistic)
      and specific OS reassembly strategy (could not be verified practically) \\
    - NTP 'prime-the-pump' \cite{malhotra_attacking_2016-1}: strongly similar to our attack, as it also abuses the rate limiting mechanism, but we use it to make the client forget the server and replace it with an attacker controlled one via DNS \\

DNS cache poisoning \\
    - prequisites for DNS cache poisoning in Section \ref{sec:attack} \\
    
\end{mytodoenv}



==> typos.tex <==
#303B
-----

* Why the results of vulnerable resolvers in residential networks (§VIII.B) are missing? It is the key to
demonstrate if the attacks can be prevalent. Intuitively, the caching state of pool.ntp.org could be
significantly higher than the state in open resolvers, since those resolvers in residential networks
would be largely used by normal clients.

#303D
-----



#303E
-----


Noted
-----

* The "attack duration" in Table II is unclear. According to the paper, it seems to be configured by the
NTP software, but in two scenarios the NTPd has different values.
* The sentence at the end of §V.A seems broken and hard to understand (i.e., P1 and P2).
[Abstract] The paper is much better than this poor Abstract, I suggest you revise/rewrite carefully to
truly reflect your contribution
[Introduction] The last paragraph of the subsection “Our attack” is repeated in the Introduction. Please
revise.

Fixed
-----

* Ref. [32] is not completed.
* In §V.A.2, "A special case is ntpdate, ... and then exists, so that there is no run-time at all."exists --> then exits?
then
[Introduction] “ognore” → “ignore”
[Abstract] I suggest you replace MitM by Man-in-the-Middle here
[Introduction] Please revise: “client queries time from multiple NTP servers” [Introduction] “or
majority” → “or a majority”
[Introduction] “which Chronos client” → “which the Chronos client”
[Introduction] “shows that NTP ecosystem” → “shows that the NTP ecosystem” (other similar errors
appear frequently throughout the paper, lack of the article “the”, I will not list the others, revise
carefully)
[Introduction] “even 500 byte fragment” → “even a 500-byte fragment”
[Section 2] “please expand the acronym KoD”
[Section 5] “and then exists” → “and then exits”
[Section 8] “namserver, all clients well be” → “nameserver, all clients are”
[Section 9] “we provide discuss” → “provide a discussion on”
[References] References [7] and [28] are the same, repeated
 - “ip”, “ntp” → convert always to capital letters
 - Section IV-B-2, ‘the attackers real address’ -> ‘the attacker’s real address’.
 - first paragraph in Section VI, ‘a internet standard document’ -> ‘an internet standard document’.
 - Section VI-A, ‘the are only done’ -> ‘they are only done’.
 - Section VII-A, ‘well be’ -> ‘will be’, ‘to not’ -> ‘do not’.

General
-------

 - lack of the article “the”, I will not list the others, revise carefully
 -  "a" -> "an"
 - ...s -> ...'s



NTP-over-DNS changes
====================

Philipp
-------

[boot-time attack] [Doing] We briefly describe (2) and (3) next and will add an explanation as well as our SMTP measurements to the manuscript.

    I'll take this from dns-attack-surface then and add the explanation from the rebuttal into the paper.
    
Done
----

[Nameserver MTU] [DONE, MEEEH] Our measurements of the minimum MTU in nameservers are as follows (we will also add to the paper)

    I'll take this from dns-attack-surface, but try to keep it short
    (no graphs, only small description how it is done).

[Evaluation analysis] [DONE] Add an explanation and more examples of different configurations and their implications for NTP clients.

    I'll add some configuration examples of default configs into the text.

[Often cached] [DONE]. Second, via a measurement study we found that the resolvers are used by different services concurrently, e.g., NTP server, Web and Email server (we will add explanation to paper)

    I'll take this from dns-attack-surface, but we only have this for sharing resolvers between web-client and SMTP servers, this does not directly relate to NTP.
    




